FinEvo: From Isolated Backtests to Ecological Market Games for Multi-Agent Financial Strategy Evolution

Conventional financial strategy evaluation relies on isolated backtests in static environments. Such evaluations assess each policy independently, overlook correlations and interactions, and fail to explain why strategies ultimately persist or vanish in evolving markets. We shift to an ecological perspective, where trading strategies are modeled as adaptive agents that interact and learn within a shared market. Instead of proposing a new strategy, we present FinEvo, an ecological game formalism for studying the evolutionary dynamics of multi-agent financial strategies. At the individual level, heterogeneous ML-based traders-rule-based, deep learning, reinforcement learning, and large language model (LLM) agents-adapt using signals such as historical prices and external news. At the population level, strategy distributions evolve through three designed mechanisms-selection, innovation, and environmental perturbation-capturing the dynamic forces of real markets. Together, these two layers of adaptation link evolutionary game theory with modern learning dynamics, providing a principled environment for studying strategic behavior. Experiments with external shocks and real-world news streams show that FinEvo is both stable for reproducibility and expressive in revealing context-dependent outcomes. Strategies may dominate, collapse, or form coalitions depending on their competitors-patterns invisible to static backtests. By reframing strategy evaluation as an ecological game formalism, FinEvo provides a unified, mechanism-level protocol for analyzing robustness, adaptation, and emergent dynamics in multi-agent financial markets, and may offer a means to explore the potential impact of macroeconomic policies and financial regulations on price evolution and equilibrium.

==> sections/0.tex <==
%Traditional financial strategy evaluation often relies on isolated backtesting in static environments, ignoring the inherently interactive and adversarial nature of real-world markets. In this work, we propose a paradigm shift: strategies should be evaluated as agents in an ecological game, where their performance emerges through repeated interactions with diverse opponents. We introduce a multi-agent simulation framework that models trading strategies—such as trend-following, contrarian, fundamentalist, and event-driven—as behavioral agents operating in a shared market. Through extensive experiments, we analyze long-term dynamics, relative payoffs, and survival patterns under different strategy combinations. Our results reveal that some strategies thrive only in the presence of others, while certain dominant behaviors suppress alternatives, leading to ecological imbalance or equilibrium. This work lays the foundation for a new class of interaction-aware evaluation benchmarks, reframing financial intelligence as a game-theoretic and ecological phenomenon rather than a static optimization problem.

%Conventional approaches to financial strategy evaluation rely on isolated backtesting or static learning environments, overlooking the inherently interactive, adaptive, and ecological dynamics of real markets. We propose a paradigm shift: financial strategies should be assessed as agents embedded in an ecological game, where their performance and survival emerge through continual interaction, competition, and adaptation among diverse participants. We present a modular agent-based simulation framework in which heterogeneous trader agents—spanning trend-following, contrarian, fundamentalist, event-driven, random, and adaptive behaviors—jointly evolve within a dynamically clearing synthetic market. The evolution of strategy composition is governed by a stochastic discrete-time Lotka–Volterra process, enabling principled modeling of selection, innovation, and ecological feedback. Through systematic experiments, we demonstrate that the effectiveness, stability, and risk profile of trading strategies are fundamentally context-dependent: many policies succeed or fail only in the presence of particular competitors or collaborators, while emergent phenomena such as dominance cycles, regime shifts, and extinction cascades remain invisible in conventional evaluations. Our work reframes financial strategy evaluation as an ecological, interaction-driven process governed by evolutionary dynamics, opening new directions for the development of robust, adaptive, and context-aware financial age

==> sections/1.1.tex <==
Financial markets are among the most complex and adaptive systems in the real world. The success or failure of any trading strategy depends not only on market signals, but critically on the collective actions and evolving behaviors of countless other participants. Despite this fundamental interdependence, most existing approaches to financial strategy evaluation---including traditional backtesting and reinforcement learning---assess performance in isolation, implicitly assuming stationary environments and passive price dynamics.

This isolated paradigm diverges sharply from reality: strategies in actual markets continuously interact, adapt, and compete for profit. The viability of a trend-following agent, for example, may hinge on the simultaneous presence of momentum chasers or mean-reversion traders; some strategies persist only when others coexist, while dominant ones may destabilize or extinguish their rivals. These ecological dependencies, which shape real-world performance, are largely invisible in conventional single-agent or static-environment evaluations.

In this work, we argue for a paradigm shift: **financial strategies should be evaluated as agents embedded within an ecological game**---a multi-agent system where performance is endogenously determined by recurrent interaction, competition, and adaptation. Rather than optimizing against a fixed, non-reactive environment, we propose to analyze the population dynamics, survival, and systemic impact of diverse strategies within a unified agent-based simulation. This ecological perspective draws on the principles of evolutionary game theory and complex systems science, promising a richer understanding of collective intelligence and market adaptation.

To operationalize this vision, we develop a flexible simulation framework in which a heterogeneous population of trader agents---each governed by a distinct, parameterized policy---jointly evolves within a shared synthetic market. The environment supports a broad taxonomy of behavioral archetypes, including trend followers, contrarians, fundamentalists, event-driven, random, and adaptive agents, each initialized with strategy-specific parameters and capital constraints. The market price emerges from the real-time clearing of all submitted buy/sell/hold orders, incorporating endogenous feedback and exogenous shocks.

Our ecological framework formalizes strategy population dynamics via a generalized Lotka–Volterra process, bridging classical evolutionary theory and modern agent-based modeling. Agents adapt, go bankrupt, or are replaced through a combination of fitness-driven selection and innovation (mutation), inducing complex ecosystem-level phenomena such as dominance cycles, regime shifts, extinction cascades, and ecological equilibria. This approach enables us to move beyond static optimization, offering a systematic methodology for benchmarking and understanding financial decision-making under realistic market interaction.

Empirically, our study reveals that the effectiveness and survival of trading strategies are highly context-dependent: many policies thrive only in the presence of specific opponents or collaborators; ecological feedback can stabilize, destabilize, or fundamentally reshape market outcomes; and naive, isolated evaluations often misjudge the true resilience or fragility of candidate strategies. By quantifying both individual and system-level metrics---including profit, risk, survival, diversity, and interaction sensitivity---our work provides a robust, reproducible foundation for future research in agent-based financial intelligence.

In summary, we contribute:
\begin{enumerate}
    \item A game-theoretic reframing of financial strategy evaluation as ecological multi-agent interaction;
    \item A modular, extensible agent-based market simulation framework supporting diverse strategy classes and population dynamics;
    \item A systematic analysis of emergent behaviors and interaction-induced phenomena in complex financial ecosystems.
\end{enumerate}
We believe that this ecological game-theoretic perspective opens new directions for the development and evaluation of robust, adaptive, and context-aware financial agents.



==> sections/1.tex <==

Financial markets are among the most complex and adaptive systems in the real world. The success or failure of any trading strategy depends not only on market signals, but critically on the collective actions and evolving behaviors of countless other participants. Despite this fundamental interdependence, most existing approaches to financial strategy evaluation---including traditional backtesting and reinforcement learning---assess performance in isolation, implicitly assuming stationary environments and passive price dynamics.

This isolated paradigm diverges sharply from reality: strategies in actual markets continuously interact, adapt, and compete for profit. The viability of a trend-following agent, for example, may hinge on the simultaneous presence of momentum chasers or mean-reversion traders; some strategies persist only when others coexist, while dominant ones may destabilize or extinguish their rivals. These ecological dependencies, which shape real-world performance, are largely invisible in conventional single-agent or static-environment evaluations.

In this work, we argue for a paradigm shift: **financial strategies should be evaluated as agents embedded within an ecological game**---a multi-agent system where performance is endogenously determined by recurrent interaction, competition, and adaptation. Rather than optimizing against a fixed, non-reactive environment, we propose to analyze the population dynamics, survival, and systemic impact of diverse strategies within a unified agent-based simulation. This ecological perspective draws on the principles of evolutionary game theory and complex systems science, promising a richer understanding of collective intelligence and market adaptation.

To operationalize this vision, we develop a flexible simulation framework in which a heterogeneous population of trader agents---each governed by a distinct, parameterized policy---jointly evolves within a shared synthetic market. The environment supports a broad taxonomy of behavioral archetypes, including trend followers, contrarians, fundamentalists, event-driven, random, and adaptive agents, each initialized with strategy-specific parameters and capital constraints. The market price emerges from the real-time clearing of all submitted buy/sell/hold orders, incorporating endogenous feedback and exogenous shocks.

Our ecological framework formalizes strategy population dynamics via a generalized Lotka–Volterra process, bridging classical evolutionary theory and modern agent-based modeling. Agents adapt, go bankrupt, or are replaced through a combination of fitness-driven selection and innovation (mutation), inducing complex ecosystem-level phenomena such as dominance cycles, regime shifts, extinction cascades, and ecological equilibria. This approach enables us to move beyond static optimization, offering a systematic methodology for benchmarking and understanding financial decision-making under realistic market interaction.

Empirically, our study reveals that the effectiveness and survival of trading strategies are highly context-dependent: many policies thrive only in the presence of specific opponents or collaborators; ecological feedback can stabilize, destabilize, or fundamentally reshape market outcomes; and naive, isolated evaluations often misjudge the true resilience or fragility of candidate strategies. By quantifying both individual and system-level metrics---including profit, risk, survival, diversity, and interaction sensitivity---our work provides a robust, reproducible foundation for future research in agent-based financial intelligence.

In summary, we contribute:
\begin{enumerate}
    \item A game-theoretic reframing of financial strategy evaluation as ecological multi-agent interaction;
    \item A modular, extensible agent-based market simulation framework supporting diverse strategy classes and population dynamics;
    \item A systematic analysis of emergent behaviors and interaction-induced phenomena in complex financial ecosystems.
\end{enumerate}
We believe that this ecological game-theoretic perspective opens new directions for the development and evaluation of robust, adaptive, and context-aware financial agents.

==> sections/2.1.tex <==
\section{Ecological Games: Problem Formulation}

We formalize financial strategy evaluation as an ecological game, where a fixed population of $N$ heterogeneous trader agents---each governed by a distinct trading policy---interacts and evolves within a shared, dynamically changing market environment. This perspective enables not only the assessment of individual strategies, but also the investigation of collective adaptation, competitive dynamics, and emergent market phenomena.

\paragraph{Agent Behavior and Market Feedback.}
At each discrete time $t$, agent $i$ holds capital $C_i^t$ and position $S_i^t$, and selects a trading action $a_i^t$ (e.g., buy, sell, hold) according to its assigned strategy $\pi_{k(i)}$ and observed market state. The market price $P_t$ is updated through a market-clearing function:
\begin{equation}
P_{t+1} = F(P_t, \{a_i^t\}_{i=1}^N, \xi_t)
\end{equation}
where $F$ aggregates all agent actions and $\xi_t$ models exogenous shocks. Each agent's portfolio is updated as:
\begin{equation}
\begin{aligned}
C_i^{t+1} &= C_i^t - a_i^{t,\text{buy}} P_t + a_i^{t,\text{sell}} P_t \\
S_i^{t+1} &= S_i^t + a_i^{t,\text{buy}} - a_i^{t,\text{sell}}
\end{aligned}
\end{equation}
Profits and losses are entirely endogenous, shaped by the joint behavior of all agents.


\paragraph{Ecological Population Dynamics.}


In practice, our simulation implements a discrete-time version of these population dynamics. At each round, the mean empirical payoff for each strategy is
\begin{equation}
f_k^t[\text{emp}] = \frac{1}{N_k^t} \sum_{i:\pi_{k(i)} = \pi_k} \left[ (C_i^{t+1} + S_i^{t+1} P_{t+1}) - (C_i^t + S_i^t P_t) \right]
\end{equation}

The performance of a learning AI agent—whether a reinforcement learning (RL) agent or a large language model (LLM)—is inherently characterized by exploration and stochastic fluctuations. For instance, an RL agent may experience unexpected high or low returns as a consequence of exploration, while an LLM's outputs may vary due to different reasoning trajectories such as chain-of-thought processes.

To rigorously capture this intrinsic variability associated with learning agents, we model the strategy reward \( f_k(t) \) as a stochastic process. Specifically, we adopt the Ornstein--Uhlenbeck (OU) process, which is well-suited for representing mean-reverting dynamics with noise. The temporal evolution of \( f_k \) is thus governed by the following stochastic differential equation (SDE):
\begin{equation}
    df_k(t) = \lambda_k \left( \bar{f}_k(E) - f_k(t) \right) \, dt + \nu_k \, dW_k(t)
\end{equation}
where \(\bar{f}_k(E)\) is the long-term expected reward of strategy \(\pi_k\) in environment \(E\); \(\lambda_k > 0\) is the learning stability parameter controlling the rate of mean reversion; \(\nu_k\) is the noise intensity representing intrinsic randomness; and \(dW_k(t)\) represents the intrinsic stochasticity of the learning dynamics, and is assumed to be independent of $dW_k(t)$, which accounts for exogenous market fluctuations.

A direct consequence of this modeling is that, at steady state, the variance of a learning AI’s reward is determined by its learning parameters:
\begin{equation}
    \text{Var}(f_k^t) = \mathbb{E} \left[ (f_k^t - \bar{f}_k^t)^2 \right] = \frac{\nu_k^2}{2\lambda_k}
\end{equation}
The dynamic evolution of trading strategy composition in our agent-based market can be theoretically described by a generalized  Stochastic Replicator-Mutator Equation :


\begin{equation}
dx_k(t) = 
\underbrace{x_k(t) \left( f_k(t) - \bar{f}(t) \right) dt}_{\text{Performance Pressure}}
+ \underbrace{\mu (m - x_k(t)) dt}_{\text{Social Adaptation}}
+ \underbrace{x_k(t) \left( \sigma_k dW_k(t) - \sum_j x_j(t) \sigma_j dW_j(t) \right)}_{\text{Environmental Drift}}
\end{equation}
% where $x_k$ denotes the fraction of agents using strategy $\pi_k$, $r_k(E)$ is the intrinsic (potentially environment-dependent) growth rate, $\gamma_{kj}(E)$ represents direct ecological interactions, $D_k(E)$ models spatial or structural heterogeneity, and $\sigma_k(E)\,\eta_k(t)$ captures random shocks.
Here, $f_k(t)$ denotes the instantaneous reward (or fitness) of strategy $k$, and the population-average reward is given by $\bar{f}(t) = \sum_j x_j(t) f_j(t)$. The first term corresponds to the classical replicator dynamics, where strategies with above-average fitness increase their population share.The second term represents the innovation or mutation effect, driving the population proportions toward a baseline distribution $m_k$ at a rate $\mu$.The third term captures population-level stochasticity arising from external market shocks. Here, $dW_k(t)$ are independent Wiener process increments. This term is constructed to ensure that, even in the presence of noise, the population proportions remain normalized, i.e., $\sum_k dx_k(t) = 0$.

By applying the Euler–Maruyama method to the above stochastic differential equation (SDE), we establish a formal connection between the continuous-time analytical framework and its discrete-time simulation counterpart.
Assume a time step size of $\Delta t = 1$, and approximate the Brownian motion increment $dW_k(t)$ by $\eta_k^t \sqrt{\Delta t}$, where $\eta_k^t \sim \mathcal{N}(0, 1)$.

The discrete-time update of $x_k^{t+1} - x_k^t$ is then given by:

\begin{equation}
x_k^{t+1} \approx x_k^t + x_k^t (f_k^t - \bar{f}^t) + \mu (m_k - x_k^t) + x_k^t (\sigma_k \eta_k^t - \bar{\eta}^t)
\end{equation}
In our simulation, agents whose capital falls below a threshold are eliminated. Replacements are then sampled via fitness-proportionate reproduction or, with a small probability $\mu$, via mutation from a base distribution $m_k$.

While a direct discretization of the governing stochastic differential equation (SDE) yields a linear approximation, the principle of fitness-proportionate reproduction is more robustly captured by an exponential (or softmax) update rule. This form is standard in evolutionary dynamics simulations as it inherently ensures that strategy proportions remain non-negative and sum to one.

Therefore, our simulation adopts the following discrete-time update rule for the population share of each strategy (see Appendix~A.1 for a detailed derivation):

\begin{equation}
\boxed{
x_k^{t+1} = (1-\mu) \frac{x_k^t \exp[\beta f_k^t + \sigma_k \eta_k^t]}
{\sum_{j} x_j^t \exp[\beta f_j^t + \sigma_j \eta_j^t]}
+ \mu\, m_k
}
\end{equation}
where $\beta$ is the selection intensity, $\sigma_k$ the noise strength, and $\eta_k^t \sim \mathcal{N}(0, 1)$.

This unified modeling perspective enables us to bridge continuous-time ecological theory and practical agent-based simulation, supporting both theoretical analysis and empirical experiments of collective intelligence in financial markets.



\subsection{Core Assumptions}
\textbf{Timescale Separation.}
We assume a separation of timescales between the reward dynamics of AI strategies, denoted by $f_k(t)$, and the population proportions $x_k(t)$. Specifically, the dynamics of $f_k(t)$—modeled as an Ornstein–Uhlenbeck (OU) process—are much faster than those of $x_k(t)$, i.e., $\lambda_k \gg 1$. This allows us to treat $f_k^t$ as having reached its stationary distribution when analyzing the one-step change $\Delta x_k$, and to approximate its variance by the steady-state value:
\[
\operatorname{Var}(f_k) = \frac{\nu_k^2}{2\lambda_k}.
\]

\textbf{Independence of Stochastic Sources.}
We assume that the three main sources of randomness are mutually independent:
\begin{itemize}
    \item The intrinsic stochasticity of AI learning, represented by $dW_k'(t)$,
    \item The external market shocks, represented by $dW_k(t)$,
    \item The innovation or introduction process of new strategies.
\end{itemize}
This assumption ensures that cross terms vanish in expectation when computing the total variance.

\textbf{Homogeneity and Independence of Shocks.}
For analytical simplicity, we assume that external shock intensity is homogeneous across all strategies, i.e., $\sigma_k = \sigma$. Additionally, we assume that at any given time $t$, the shocks $\eta_k^t$ affecting different strategies are independently and identically distributed (i.i.d.) as standard normal variables: $\eta_k^t \sim \mathcal{N}(0,1)$.

\subsection{AI market volatility}
To analyze the sources of population variance, we decompose the variance of $\Delta x_k$
into three components corresponding to selection, noise, and innovation, respectively.We perform a first-order approximation of the population update rule.

\begin{equation}
\Delta x_k \approx \underbrace{x_k^t \cdot \beta \left(f_k^t - \bar{f}^t \right)}_{\text{selection}} + \underbrace{x_k^t \cdot \left( \sigma \eta_k^t - \sigma \bar{\eta}^t \right)}_{\text{noise}} + \underbrace{\mu (m_k - x_k^t)}_{\text{innovation}}
\end{equation}
We compute the expectation of \((\Delta x_k)^2\).Under Assumption 2, the cross terms vanish in expectation. Therefore, it suffices to calculate the expectation of the square of each individual term:
\begin{equation}
    \mathbb{E}\left[ (\Delta x_k)^2 \right] \approx 
\mathbb{E}\left[ (\text{selection})^2 \right] + 
\mathbb{E}\left[ (\text{noise})^2 \right] + 
\mathbb{E}\left[ (\text{innovation})^2 \right]
\end{equation}

The expectation of the squared innovation term is given by

\[
\mathbb{E}[(\text{select})^2] = \mathbb{E}\left[ \left( x_k^t \beta (f_k^t - \bar{f}^t) \right)^2 \right] = (x_k^t \beta)^2 \, \mathbb{E}\left[ (f_k^t - \bar{f}^t)^2 \right].
\]
Under Assumption~1 (Timescale Separation), the stationary variance of $f_k$ can be used in the analysis:
\[
\mathbb{E}[(\text{select})^2] = (x_k^t \beta)^2 \mathrm{Var}(f_k) = (x_k^t \beta)^2 \left( \frac{\nu_k^2}{2 \lambda_k} \right).
\]

\[
\mathbb{E}[(\text{innovate})^2] = \mu^2 (m_k - x_k^t)^2.
\]

The expected variance of this term can be calculated precisely, quantifying how external shocks are translated into volatility through the population structure. Its specific mathematical derivation is rather lengthy and has been included in Appendix A.1.
\[
\mathbb{E}[(\text{noise})^2] = \sigma^2 (x_k^t)^2 \left( 1 - 2 x_k^t + \| x^t \|_2^2 \right).
\]

The AI market volatility at time \(t\), denoted by \(V_{\mathrm{AI}}^t\), can be approximated as the sum of the three driving components:

\[
V_{\mathrm{AI}}^t \approx V_{\text{select}} + V_{\text{noise}} + V_{\text{innovate}}.
\]
This term directly arises from the intrinsic learning characteristics of AI agents and measures the AI market volatility driven by the inherent uncertainty in AI strategy performance.
\begin{equation}
    V_{\text{select}} = \beta^2 \sum_k \left( x_k^t \right)^2 \cdot \left( \frac{\nu_k^2}{2\lambda_k} \right)
\end{equation}
This term represents the AI market volatility induced by random shocks from the external market environment.
\begin{equation}
    V_{\text{noise}} = \sigma^2 \sum_k (x_k^t)^2 \left( 1 - 2 x_k^t + \| x^t \|_2^2 \right)
\end{equation}
This term captures the impact of continual influx of new strategies on the existing market ecosystem.
\begin{equation}
    V_{\text{innovation}} = \mu^2 \sum_k (m_k - x_k^t)^2
\end{equation}

\paragraph{Research Questions.}
This ecological game-theoretic formalism enables us to address fundamental research questions:
\begin{itemize}
    \item \textbf{Survival and dominance:} Which strategies persist, expand, or vanish under different market ecologies?
    \item \textbf{Ecological dependencies:} How do interactions between strategies modulate market stability and agent viability?
    \item \textbf{Emergent equilibria:} What conditions lead to stabilization, oscillation, or collapse of population structure?
    \item \textbf{Robustness and innovation:} How do adaptation, mutation, and strategy diversity impact the resilience of the agent ecosystem?
\end{itemize}
Grounded in evolutionary and ecological dynamics, our framework transcends static optimization, enabling holistic and interaction-aware analysis of financial intelligence in complex markets.


==> sections/2.2.tex <==


\section{Ecological Games: Problem Formulation}

We cast financial strategy evaluation as an \emph{ecological game}, where a population of $N$ heterogeneous trader agents—each governed by a distinct trading policy—interacts and adapts within a shared, dynamically evolving market. This lens supports assessing individual strategies while analyzing collective adaptation, competitive dynamics, and emergent patterns.

\paragraph{Agent Behavior and Market Feedback.}
At each discrete time $t$, agent $i$ holds capital $C_i^t$ and position $S_i^t$, and selects $a_i^t \in \{\text{buy}, \text{sell}, \text{hold}\}$ according to its policy $\pi_{k(i)}$ and the market state. The market price updates through a clearing function that aggregates all actions and exogenous shocks:
\begin{equation}
P_{t+1} = F\!\big(P_t,\{a_i^t\}_{i=1}^N,\xi_t\big),
\end{equation}
and portfolios evolve as
\begin{equation}
\begin{aligned}
C_i^{t+1} &= C_i^t - a_i^{t,\text{buy}} P_t + a_i^{t,\text{sell}} P_t,\\
S_i^{t+1} &= S_i^t + a_i^{t,\text{buy}} - a_i^{t,\text{sell}}.
\end{aligned}
\end{equation}
Profits and losses are endogenous to joint actions.

\paragraph{Stochastic Strategy Payoffs.}
For strategy $\pi_k$, the empirical (sample) mean payoff over $[t,t{+}1]$ is
\begin{equation}
\hat{f}_k^t
= \frac{1}{N_k^t} \sum_{i:\,\pi_{k(i)}=\pi_k}
\left[ C_i^{t+1} + S_i^{t+1} P_{t+1} - \big(C_i^{t} + S_i^{t} P_{t}\big) \right],
\end{equation}
where $N_k^t$ is the number of agents using $\pi_k$ at time $t$.
We model the \emph{instantaneous} (latent) payoff $f_k(t)$ as an Ornstein--Uhlenbeck (OU) process,
\begin{equation}
df_k(t) = \lambda_k\big(\theta_k(E) - f_k(t)\big)\,dt + \nu_k\, dB_k(t),
\end{equation}
With long-run mean $\theta_k(E)$, mean-reversion rate $\lambda_k>0$, noise intensity $\nu_k$, and ${B_k(t)}_k$ independent Wiener processes (independent of market shocks and across $k$), the OU specification is appropriate because competition induces reversion of excess returns, learning agents (RL/LLM) generate intrinsic fluctuations, and the linear–Gaussian structure yields tractable period aggregation and estimation. At stationarity, the process satisfies $\mathbb{E}[f_k(t)]=\theta_k(E)$ and $\mathrm{Var}[f_k(t)]=\nu_k^2/(2\lambda_k)$. To align model outputs with observed data, we link the empirical mean $\hat f_k^t$ to the period-average latent payoff $\bar f_k^t = \int_t^{t+1} f_k(s)ds$ through
$\hat f_k^t = \bar f_k^t + \varepsilon_k^t$,
where $\varepsilon_k^t$ is zero-mean noise with variance decreasing in $N_k^t$.

\paragraph{Population Dynamics.}
Let $x_k(t)$ denote the fraction of agents using strategy $\pi_k$, with $\sum_k x_k(t)=1$.  
The continuous-time evolution follows a stochastic replicator--mutator equation:
\begin{equation}
dx_k(t) =
\underbrace{x_k(t) \big( f_k(t) - \bar{f}(t) \big) dt}_{\text{Performance Pressure}}
+ \underbrace{\mu \big( m^t - x_k(t) \big) dt}_{\text{Social Adaptation}}
+ \underbrace{x_k(t) \Big( \sigma_k\, dW_k(t) - \sum_j x_j(t)\, \sigma_j\, dW_j(t) \Big)}_{\text{Environmental Drift}},
\end{equation}

where $\bar f(t)=\sum_{j} x_j(t)\, f_j(t)$ is the population-average payoff,  
$\mu \ge 0$ is the mutation rate, the target distribution of mutation/adaptation 
$m^{t}$ is drawn from a Dirichlet distribution: 
$m^{t} \sim \mathrm{Dir}(\alpha_1, \alpha_2, \ldots, \alpha_K)$,
where $\alpha_k > 0$ are the concentration parameters.
The processes $\{W_k(t)\}_k$ are independent standard Wiener processes (taken independent of $\{B_k(t)\}_k$).  
The noise term is written in simplex-tangent form, ensuring $\sum_k dx_k(t)=0$ and thus preserving $\sum_k x_k(t) \equiv 1$.

For implementation, we use a discrete-time update derived in Appendix~\S A, obtained by applying a one-step multiplicative-weights selection flow, followed by mutation mixing and logit-normal shocks—yielding a first-order correspondence to the replicator drift.


\paragraph{Core assumptions and volatility.}
We assume a fast--slow separation: the OU payoff $f_k(t)$ relaxes quickly ($\lambda_k \gg 1$), allowing $x(t)$ to be treated as quasi-static over a single step, with $f_k(t)$ near stationarity and $\mathrm{Var}(f_k)=\nu_k^2/(2\lambda_k)$. Randomness from payoff noise $dB_k(t)$, environmental shocks $dW_k(t)$, and the innovation mechanism (rate $\mu$, baseline $m$) is taken to be mutually independent. For tractability, we use homogeneous shock intensity $\sigma_k=\sigma$ and i.i.d.\ discrete shocks $\eta_k^t \sim \mathcal{N}(0,1)$. A first--order step consistent with the earlier SDE decomposes as
\[
\Delta x_k \approx 
\beta x_k^t (f_k^t - \bar{f}^t) 
+ \mu (m_k^t - x_k^t) 
+ x_k^t (\sigma \eta_k^t - \bar{\sigma \eta}^t)
\]

where $\bar f^t=\sum_j x_j^t f_j^t$ and $\bar\eta^t=\sum_j x_j^t \eta_j^t$.  

The corresponding per--step variance for strategy $k$ is simply the sum of three contributions: performance pressure, social adaptation, and environmental drift,
\[
\mathrm{Var}(\Delta x_k) \approx 
\beta^2 (x_k^t)^2 \frac{\nu_k^2}{2\lambda_k}
+ \mu^2 \frac{m_k(1-m_k)}{\alpha_0 + 1}
+ \sigma^2 (x_k^t)^2 \big( 1 - 2x_k^t + \|x^t\|_2^2 \big),
\]
where $\|x^t\|_2^2=\sum_j (x_j^t)^2$.

Aggregating over $k$ gives the total volatility indicator
\begin{equation}
\begin{aligned}
V_{\mathrm{AI}}^t &= V_{\text{Performance Pressure}}^t + V_{\text{Social Adaptation}}^t + V_{\text{Environmental Drift}}^t \\[2pt]
&= \beta^2 \sum_k (x_k^t)^2 \frac{\nu_k^2}{2\lambda_k}
  + \mu^2\sum_k \frac{m_k (1 - m_k)}{ \alpha_0 + 1} 
  + \sigma^2 \sum_k (x_k^t)^2 \big( 1 - 2 x_k^t + \| x^t \|_2^2 \big).
\end{aligned}
\end{equation}





\paragraph{Research Questions.}
This ecological game-theoretic formalism enables us to address fundamental research questions:
\begin{itemize}
    \item \textbf{Survival and dominance:} Which strategies persist, expand, or vanish under different market ecologies?
    \item \textbf{Ecological dependencies:} How do interactions between strategies modulate market stability and agent viability?
    \item \textbf{Emergent equilibria:} What conditions lead to stabilization, oscillation, or collapse of population structure?
    \item \textbf{Robustness and innovation:} How do adaptation, mutation, and strategy diversity impact the resilience of the agent ecosystem?
\end{itemize}
Grounded in evolutionary and ecological dynamics, our framework transcends static optimization, enabling holistic and interaction-aware analysis of financial intelligence in complex markets.

==> sections/2.3.tex <==
\section{Ecological Games: Problem Formulation}

We cast financial strategy evaluation as an \emph{ecological game}, where a population of $N$ heterogeneous trader agents—each governed by a distinct trading policy—interacts and adapts within a shared, dynamically evolving market. This lens supports assessing individual strategies while analyzing collective adaptation, competitive dynamics, and emergent patterns.

\paragraph{Agent Behavior and Market Feedback.}  
At each discrete time $t$, agent $i$ holds capital $C_i^t$ and position $S_i^t$.  
Its action $a_i^t \in \{\text{buy}, \text{sell}, \text{hold}\}$ is drawn according to policy $\pi_{k(i)}$, which conditions on both the recent price history and exogenous news signals, while the market price evolves as a function of all actions and residual shocks:
\begin{equation}
a_i^t \sim \pi_{k(i)}\!\big(\{P_{t-\tau},\dots,P_t\}, E_t\big),
\qquad
P_{t+1} = F\!\big(P_t, \{a_i^t\}_{i=1}^N, \xi_t\big),
\end{equation}
where $\xi_t$ represents residual market noise.  

Finally, portfolios update according to executed trades:
\begin{equation}
C_i^{t+1} = C_i^t - a_i^{t,\text{buy}} P_t + a_i^{t,\text{sell}} P_t,
\qquad
S_i^{t+1} = S_i^t + a_i^{t,\text{buy}} - a_i^{t,\text{sell}}.
\end{equation}

In this formulation, actions are directly shaped by past market information and exogenous drivers, while prices are an endogenous outcome of the collective set of actions, closing the feedback loop between agent decisions and market dynamics.


\paragraph{Forward-looking Strategy Value.}
For strategy $\pi_k$, the realized payoff over $[t,t{+}1]$ is
\[
\hat{f}_k^t = \frac{1}{N_k^t} \sum_{i:\,\pi_{k(i)}=\pi_k}
\big[ C_i^{t+1} + S_i^{t+1} P_{t+1} - (C_i^{t} + S_i^{t} P_t) \big],
\]
representing the \emph{instantaneous reward} observed from trading. 

Analogous to reinforcement learning, where agents estimate a value function beyond immediate rewards, we let $V_k(t)$ denote the \emph{forward-looking value} of $\pi_k$. This value reflects expected future performance, anchored to an environment-conditioned mean payoff $f_k(E_t)$—akin to a dynamic target shaped by external signals $E_t$ (e.g., macro news, policy shifts).

We model $V_k(t)$ via an Ornstein--Uhlenbeck (OU) process:
\[
dV_k(t) = \lambda_k\big(f_k(E_t) - V_k(t)\big)\,dt + \nu_k\,dB_k(t),
\]
where $\lambda_k>0$ governs the adjustment speed toward the target $f_k(E_t)$, $\nu_k>0$ controls exploration-like noise, and $B_k(t)$ is a standard Wiener process independent across strategies. 

This mirrors temporal-difference learning in RL: $\hat f_k^t$ plays the role of the immediate reward, $f_k(E_t)$ acts as the moving target value, and $V_k(t)$ continually updates toward it. Such a structure allows strategies to integrate short-term outcomes with persistent market signals, providing a predictive basis for adaptive evolution.





\paragraph{Evolutionary Update Mechanism.}  
Let $x_k(t)$ denote the fraction of agents using strategy $\pi_k$, with $\sum_k x_k(t)=1$.  
The population share evolves according to a stochastic replicator--mutator equation:
\begin{equation}
dx_k(t) =
\underbrace{x_k(t)\big(V_k(t) - \bar V(t)\big)dt}_{\text{Relative Performance Pressure.}}
+ \underbrace{\mu\,(m^t - x_k(t))dt}_{\text{Innovation and Social Mixing.}}
+ \underbrace{x_k(t)\Big(\sigma_k dW_k(t) - \sum_j x_j(t)\sigma_j dW_j(t)\Big)}_{\text{Environmental Perturbation.}},
\end{equation}
where $\bar V(t) = \sum_j x_j(t) V_j(t)$ is the population-average payoff.  

Three mechanisms jointly shape adaptation:  

- \emph{Relative Performance Pressure.}  
  Strategies adjust according to their advantage $V_k(t) - \bar V(t)$, rewarding outperformance and penalizing underperformance.  
  This mirrors advantage-based updates in reinforcement learning, ensuring adaptation is comparative rather than absolute.  

- \emph{Innovation and Social Mixing.}  
  The mutation term $\mu(m^t - x_k)$ introduces exploration and prevents premature convergence.  
  The target distribution $m^t \sim \mathrm{Dir}(\alpha_1,\ldots,\alpha_K)$ captures social influence and random experimentation, reflecting how new strategies may diffuse in practice.  

- \emph{Environmental Perturbation.}  
  The noise term, written in simplex-tangent form, models exogenous shocks and endogenous uncertainty.  
  It preserves normalization ($\sum_k x_k(t)=1$) while keeping the system dynamically responsive to volatility and unforeseen events.  

Together, these three forces—performance-driven selection, innovation-driven diversification, and environment-driven perturbation—govern the evolutionary trajectory of strategies.  
For simulation, we adopt a discrete-time approximation via multiplicative-weights updating, followed by mutation mixing and logit-normal shocks.


\paragraph{Momentary Mechanisms of Evolution.}  
At each time step, the change in strategy shares $\Delta x_k$ arises from the joint influence of three mechanisms:  
(1) payoff-driven relative advantage,  
(2) innovation and social mixing, and  
(3) environmental perturbations.  
These forces interact contemporaneously to determine short-run dynamics.  

Assuming fast relaxation of $f_k(t)$ ($\lambda_k \gg 1$) and independence of shocks, a tractable discrete approximation is
\begin{equation}
\Delta x_k \approx 
\beta x_k^t\big(V_k^t - \bar V^t\big) 
+ \mu(m_k^t - x_k^t) 
+ x_k^t\big(\sigma\eta_k^t - \bar{\sigma\eta}^t\big),
\end{equation}
with $\eta_k^t \sim \mathcal{N}(0,1)$.  
The variance contribution of each mechanism can be decomposed as
\begin{equation}
\mathrm{Var}(\Delta x_k) \approx 
\underbrace{\beta^2 (x_k^t)^2 \tfrac{\nu_k^2}{2\lambda_k}}_{\text{Performance pressure}}
+ \underbrace{\mu^2 \tfrac{m_k(1-m_k)}{\alpha_0+1}}_{\text{Innovation}}
+ \underbrace{\sigma^2 (x_k^t)^2 \big(1 - 2x_k^t + \|x^t\|_2^2 \big)}_{\text{Environmental shocks}},
\end{equation}
where $\|x^t\|_2^2=\sum_j (x_j^t)^2$.  
Aggregating across strategies gives an overall volatility indicator,
\begin{equation}
V_{\mathrm{evo}}^t
= V_{\text{Selection}}^t
+ V_{\text{Innovation}}^t
+ V_{\text{Environment}}^t,
\end{equation}
which quantifies how selection, innovation, and perturbations jointly shape the short-run fluctuations of the evolving market ecology.



==> sections/2.tex <==

\section{Ecological Games: Problem Formulation}

We formalize financial strategy evaluation as an ecological game, where a fixed population of $N$ heterogeneous trader agents---each governed by a distinct trading policy---interacts and evolves within a shared, dynamically changing market environment. This perspective enables not only the assessment of individual strategies, but also the investigation of collective adaptation, competitive dynamics, and emergent market phenomena.

\paragraph{Agent Behavior and Market Feedback.}
At each discrete time $t$, agent $i$ holds capital $C_i^t$ and position $S_i^t$, and selects a trading action $a_i^t$ (e.g., buy, sell, hold) according to its assigned strategy $\pi_{k(i)}$ and observed market state. The market price $P_t$ is updated through a market-clearing function:
\begin{equation}
P_{t+1} = F(P_t, \{a_i^t\}_{i=1}^N, \xi_t)
\end{equation}
where $F$ aggregates all agent actions and $\xi_t$ models exogenous shocks. Each agent's portfolio is updated as:
\begin{equation}
\begin{aligned}
C_i^{t+1} &= C_i^t - a_i^{t,\text{buy}} P_t + a_i^{t,\text{sell}} P_t \\
S_i^{t+1} &= S_i^t + a_i^{t,\text{buy}} - a_i^{t,\text{sell}}
\end{aligned}
\end{equation}
Profits and losses are entirely endogenous, shaped by the joint behavior of all agents.


\paragraph{Ecological Population Dynamics.}
The dynamic evolution of trading strategy composition in our agent-based market can be theoretically described by a generalized stochastic Lotka–Volterra equation:
\begin{equation}
\frac{dx_k}{dt} = x_k\left(r_k(E) - \sum_j \gamma_{kj}(E)\, x_j\right)
+ \nabla \cdot \left(D_k(E)\, \nabla x_k\right) + \sigma_k(E)\, \eta_k(t),
\end{equation}
where $x_k$ denotes the fraction of agents using strategy $\pi_k$, $r_k(E)$ is the intrinsic (potentially environment-dependent) growth rate, $\gamma_{kj}(E)$ represents direct ecological interactions, $D_k(E)$ models spatial or structural heterogeneity, and $\sigma_k(E)\,\eta_k(t)$ captures random shocks.

In practice, our simulation implements a discrete-time version of these population dynamics. At each round, the mean empirical payoff for each strategy is
\begin{equation}
f_k^t = \frac{1}{N_k^t} \sum_{i:\, \pi_{k(i)} = \pi_k} \left[ (C_i^{t+1} + S_i^{t+1} P_{t+1}) - (C_i^t + S_i^t P_t) \right].
\end{equation}
Agents whose capital falls below a threshold are eliminated, and replacements are sampled via fitness-proportionate reproduction or, with probability $\mu$, via mutation from a base distribution $m_k$.

This leads to the following discrete-time update rule for the population share of each strategy (see Appendix~\ref{appendix:formula_simulation} for a detailed derivation and justification):
\begin{equation}
\boxed{
x_k^{t+1} = (1-\mu) \frac{x_k^t \exp[\beta f_k^t + \sigma_k \eta_k^t]}
{\sum_{j} x_j^t \exp[\beta f_j^t + \sigma_j \eta_j^t]}
+ \mu\, m_k
}
\end{equation}
where $\beta$ is the selection intensity, $\sigma_k$ the noise strength, and $\eta_k^t \sim \mathcal{N}(0, 1)$.

This unified modeling perspective enables us to bridge continuous-time ecological theory and practical agent-based simulation, supporting both theoretical analysis and empirical experiments of collective intelligence in financial markets.


\paragraph{Research Questions.}
This ecological game-theoretic formalism enables us to address fundamental research questions:
\begin{itemize}
    \item \textbf{Survival and dominance:} Which strategies persist, expand, or vanish under different market ecologies?
    \item \textbf{Ecological dependencies:} How do interactions between strategies modulate market stability and agent viability?
    \item \textbf{Emergent equilibria:} What conditions lead to stabilization, oscillation, or collapse of population structure?
    \item \textbf{Robustness and innovation:} How do adaptation, mutation, and strategy diversity impact the resilience of the agent ecosystem?
\end{itemize}
Grounded in evolutionary and ecological dynamics, our framework transcends static optimization, enabling holistic and interaction-aware analysis of financial intelligence in complex markets.

==> sections/3.1.tex <==

\section{Experiments and Analysis of Evolutionary Dynamics}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:setup}

To systematically investigate the ecological dynamics of financial strategies, we construct a multi-agent simulation environment and design two distinct experimental scenarios: a simulation with artificial shocks and a simulation driven by real-world news events.

\paragraph{Agent Population}
Our market ecology is populated by a heterogeneous ensemble of 20 distinct trader agent archetypes, varying in their behaviors, information sources, and decision-making logic. We categorize these agents into four primary classes:
\begin{itemize}
    \item \textbf{Rule-based Agents:} Encompassing traditional strategies such as trend-following, mean-reversion, event-driven traders, informational (fundamental) traders,and noise traders.
    \item \textbf{Deep Learning Agents:} Supervised learning models that leverage neural networks (e.g.,Informer,TimeMixer) to predict price direction based on market indicators.
    \item \textbf{Reinforcement Learning (RL) Agents:} Adaptive policies, such as DoubleDQN and PPO, that optimize their cumulative returns through online interaction with the market environment.
    \item \textbf{Large Language Model (LLM) Agents:} An emerging class of strategies that utilize LLMs to parse textual information from news and announcements, making trade decisions based on derived market sentiment and indicators,such as FinCon and TradingAgents.
\end{itemize}
The detailed design and parameterization of each agent class are provided in Appendix~\ref{app:agentlibrary}. For brevity, we will refer to these agents by their abbreviations in the following sections; a complete mapping of these abbreviations to their corresponding full names is also detailed in the above appendix.

\paragraph{Simulation Scenarios}
To ensure the robustness of our findings, each experimental scenario is subjected to extensive Monte Carlo analysis, with each configuration repeated for \textbf{256 independent runs}.
\begin{itemize}
    \item \textbf{Simulation with Artificial Shocks:} In this setting, we introduce a series of pre-defined, artificial shocks into the market to test the ecosystem's response, stability, and resilience under controlled perturbations.
    \item \textbf{Simulation with Real-World News:} This experiment simulates the period from July 2023 to July 2025. In this scenario, we connect the market to a stream of real historical news events, which allows event-driven and LLM agents to process real-world information. This enables an evaluation of strategy performance and interaction within a more realistic, unstructured information environment.
\end{itemize}

\paragraph{Analysis Metrics and Presentation}
Our analysis framework aligns with the multi-level research questions (micro, meso, and macro) posed in Section~2. We focus on evaluating the following metrics:
\begin{itemize}
    \item \textbf{Population Proportion Evolution (Micro):} We track the dynamic changes in the market share of each agent type to identify dominant and vanishing strategies.
    \item \textbf{Synergistic and Antagonistic Relationships (Meso):} By analyzing correlations between agent population shares, we dynamically uncover symbiotic (synergistic) or competitive (antagonistic) relationships. These long-term interaction patterns are visualized using a heatmap.
    \item \textbf{Volatility Decomposition (Macro):} We decompose the total variance of strategy share changes into contributions from the three core mechanisms: \textit{Relative Performance Pressure}, \textit{Innovation and Social Mixing}, and \textit{Environmental Perturbations}.
    \item \textbf{Agent Win Rate (Micro):} We measure the frequency of positive returns or a composite performance score for each agent as a supplementary indicator of its long-term viability.
\end{itemize}
To enhance the clarity of time-series visualizations and identify underlying trends, we apply a Savitzky-Golay filter to smooth the raw data for the \textit{population proportion evolution} and the \textit{three pressure volatility metrics}.

\subsection{Simulation Under Exogenous Shocks}

To systematically investigate the adaptive dynamics of the market ecology under external perturbations, we design a set of \textbf{controlled shock simulations}. In our synthetic market, we inject large-scale exogenous news shocks within a fixed time window from 12:00 to 13:30, considering two contrasting scenarios: \emph{highly positive} versus \emph{highly negative} news environments.

\paragraph{Population-Proportion Evolution under Exogenous Shocks.}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/result.jpeg}
    \caption{Temporal evolution of agent population proportions under simulated upward (left) and downward (right) shocks.}
    \label{fig:shock_results}
\end{figure}
As shown in Figure~\ref{fig:shock_results}, the injection of exogenous shocks reveals the ecosystem's complex, non-linear dynamics and its capacity for rapid regime shifts. We observe a highly \textbf{asymmetric response} to the perturbations. A positive shock dismantles the pre-existing monopoly of the CoT agent, fostering a more pluralistic and competitive environment where agents like CIT and ReAct gain significant market share. Conversely, a negative shock triggers a rapid re-concentration of power, transforming a balanced oligopoly into a new stable state dominated by a coalition of high-performing LLM agents (e.g., FinCon, ReAct). This \textbf{path dependency breaking} and the formation of new, context-dependent equilibria validate our eco-evolutionary framework's ability to capture complex emergent phenomena driven by multi-agent interaction, which would be invisible to traditional, isolated backtesting methods.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/result (6).jpeg}
    \caption{Evolution of correlation matrices under simulated upward (top) and downward (bottom) shocks.}
    \label{fig:correlation_evolution}
\end{figure}

\paragraph{Synergistic and Antagonistic Dynamics under Exogenous Shocks.}
To further understand how collective behaviors reorganize after shocks, 
Figure~\ref{fig:correlation_evolution} illustrates the temporal evolution of the 
\emph{correlation matrices} among heterogeneous trading agents under controlled 
exogenous shocks (12:00--13:30). Red regions indicate strong positive correlations, 
suggesting the formation of \emph{synergistic alliances}, whereas blue regions indicate 
strong negative correlations, corresponding to \emph{strategic antagonism}.

Across three temporal phases, distinct adaptive patterns emerge:

\begin{itemize}
    \item \textbf{Initial Phase (T=5\%)}: 
    Before the shock, several clusters of agents exhibit highly correlated behaviors 
    (large red blocks), implying that in a stable environment, diverse strategies tend 
    to converge into \emph{homogeneous coordination clusters}.
    
    \item \textbf{Impact Phase (T=50\%)}: 
    The exogenous shock disrupts the pre-existing equilibrium, causing a 
    \emph{fragmentation of alliances}. This is reflected in the partial disappearance 
    of red blocks and the emergence of blue bands, signifying increased strategic 
    competition and rapid divergence in agent behaviors.
    
    \item \textbf{Post-Shock Equilibrium (T=100\%)}: 
    After the shock, the system exhibits \emph{context-dependent alliance reformation}, 
    where new clusters of positively correlated agents emerge. Interestingly, 
    the reorganization patterns differ substantially between upward and downward 
    shocks, highlighting the \emph{path-dependent} nature of ecological adaptation 
    in financial markets.
\end{itemize}

These findings validate our eco-evolutionary framework by showing that 
\emph{market stability is closely linked to the structure of synergy--antagonism 
relations}, and that exogenous perturbations trigger an adaptive rebalancing 
process leading to new ecological steady states.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/result (7).jpeg}
    \caption{Evolution of top strategy-pair correlations under simulated upward (left) and downward (right) shocks.}
    \label{fig:key_pair_correlation}
\end{figure}

\paragraph{Stability of Synergy--Antagonism Structures.}
Zooming into the micro-level, Figure~\ref{fig:key_pair_correlation} tracks the evolution of key strategy-pair correlations under simulated upward and downward shocks. We observe that:  
(1) several pairs maintain \emph{persistent synergies} (high positive correlations),  
(2) others exhibit \emph{stable antagonisms} (high negative correlations), and  
(3) shocks induce only \emph{localized reorganization} without altering the 
underlying synergy--antagonism backbone.  

These results confirm that the market ecology is structured around a relatively 
stable coordination--competition framework, while external shocks trigger 
context-dependent adjustments.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/result (1).jpeg}
    \caption{Normalized evolution of theoretical volatility metrics under simulated upward (left) and downward (right) shocks.}
    \label{fig:volatility_metrics}
\end{figure}

\paragraph{Volatility Decomposition under Exogenous Shocks.}
Finally, to explain the underlying drivers of these adaptive dynamics, 
Figure~\ref{fig:volatility_metrics} reports the normalized evolution of three theoretical 
volatility components under simulated upward and downward shocks:  
(1) $\mathbf{V_{\mathrm{select}}}$ (blue), capturing \emph{selection pressure} induced by 
relative performance differentials;  
(2) $\mathbf{V_{\mathrm{innovate}}}$ (red), quantifying \emph{innovation pressure} that 
sustains diversity; and  
(3) $\mathbf{V_{\mathrm{noise}}}$ (green), reflecting \emph{stochastic drift} driven by 
exogenous shocks and endogenous uncertainty.

We observe distinct dynamics across scenarios:  
in the upward shock, $\mathbf{V_{\mathrm{noise}}}$ spikes during perturbation, fragmenting 
existing alliances, after which $\mathbf{V_{\mathrm{select}}}$ dominates, enabling a more 
pluralistic equilibrium; in the downward shock, a similar spike in 
$\mathbf{V_{\mathrm{noise}}}$ is followed by a sharp rise of $\mathbf{V_{\mathrm{select}}}$, 
driving rapid convergence toward a new LLM-dominated regime.  
$\mathbf{V_{\mathrm{innovate}}}$ remains relatively stable in both cases, implying its role 
as a background mechanism maintaining ecological diversity rather than directly driving regime shifts.

These results confirm the eco-evolutionary hypothesis of FinEvo:  
\emph{selection, innovation, and environmental perturbations jointly govern market adaptation, 
with exogenous shocks amplifying $\mathbf{V_{\mathrm{noise}}}$ while long-run equilibria 
are primarily shaped by $\mathbf{V_{\mathrm{select}}}$.}




\subsection{Empirical Analysis of Intra-Day Evolutionary Dynamics}
After examining the adaptive dynamics under simulated shocks, 
we next turn to \emph{real-world} data and analyze the 
\textbf{intra-day evolutionary dynamics} within a single trading day. 
This allows us to validate whether the eco-evolutionary patterns 
observed in controlled experiments persist under actual market conditions.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/real_intraday.jpeg}
    \caption{Intra-day evolution of agent population proportions (left) and theoretical volatility metrics (right) on July 5, 2025.}
    \label{fig:real_intraday}
\end{figure}

Figure~\ref{fig:real_intraday} illustrates the intra-day evolution of agent population proportions 
(left) and the decomposition of theoretical volatility metrics (right) on July 5, 2025.
We observe a highly dynamic, multi-phase ecological adaptation process that aligns 
closely with the theoretical drivers of the FinEvo framework.

\paragraph{Phase I (09:30--11:00): Early-Morning Convergence.}
A sharp rise in $\mathbf{V_{\mathrm{select}}}$ indicates strong selection pressure, 
amplifying the dominance of high-performing strategies (e.g., FinCon, Trading) 
while rapidly eliminating low-performing agents. The market temporarily 
converges toward a concentrated, near-monopolistic regime.

\paragraph{Phase II (11:00--14:00): Innovation-Sustained Diversification.}
$\mathbf{V_{\mathrm{innovate}}}$ remains persistently high, sustaining 
strategic diversity even as $\mathbf{V_{\mathrm{noise}}}$ begins to climb 
around midday. Mid-sized agents (e.g., CIT, BT, SIT) regain market share, 
and the ecosystem transitions from early convergence toward a more 
pluralistic composition.

\paragraph{Phase III (14:00--17:00): Noise-Induced Fragmentation and Rebalancing.}
In the afternoon, $\mathbf{V_{\mathrm{noise}}}$ peaks while 
$\mathbf{V_{\mathrm{select}}}$ temporarily weakens, triggering the breakdown 
of previously dominant alliances. Capital reallocates toward tactical agents 
(e.g., TimeMixer), and $\mathbf{V_{\mathrm{select}}}$ rises again before 
close, driving the system into a new regime dominated by Informer and TimeMixer..

This single-day analysis demonstrates that intra-day market ecology exhibits 
\emph{non-linear, multi-phase, and path-dependent} dynamics. Selection pressure 
drives rapid early convergence, innovation maintains diversity, and environmental 
noise induces alliance fragmentation and regime shifts. These findings validate 
FinEvo's eco-evolutionary hypothesis in real-world settings.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/intraday_correlation_matrix.png}
    \caption{Dynamic evolution of intra-day correlation matrices on July 5, 2025. 
    Red blocks represent \emph{synergistic alliances}, while blue blocks indicate 
    \emph{strategic antagonism}.}
    \label{fig:intraday_correlation}
\end{figure}
\paragraph{Dynamic Alliance Reconfiguration.}
Figure~\ref{fig:intraday_correlation} illustrates the intra-day evolution of 
agent-agent correlations, showing a dynamic interplay between 
\emph{synergistic alliances} and \emph{strategic antagonisms}. 
The market initially features multiple competing clusters with strong internal 
coordination, which are subsequently fragmented and reorganized under rising 
environmental noise. Toward the close, these transient shifts consolidate into 
a new regime characterized by restructured alliances and altered power balances. 
Overall, the intra-day dynamics reveal a \emph{non-stationary synergy--antagonism 
structure}, where external shocks and internal selection pressures jointly drive 
continuous ecological reorganization.

\paragraph{Performance Rankings in Bull vs. Bear Markets}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/winrate.jpeg}
    \caption{Agent Performance Rankings in Bull vs. Bear Markets. }
    \label{fig:winrate_bull_bear}
\end{figure}

We approximate January--October 2022 as a \emph{bear market phase}, 
objectively defined by persistent downward dynamics in the synthetic environment, 
and October 2024--July 2025 as a \emph{bull market phase}, characterized by 
sustained recoveries and new highs. 
Figure~\ref{fig:winrate_bull_bear} compares podium finishes and 
top-3 win rates across these regimes.

Our analysis shows that agent performance is highly \textbf{regime-dependent} 
: bull markets produce a concentrated dominance by a few strategies
, whereas bear markets foster a more dispersed competitive landscape
Notably, \textbf{LLM-based agents consistently rank higher across both regimes}
This suggests that their ability to integrate diverse informational cues and adapt flexibly
confers a significant robustness advantage over strategies based on fixed rules or purely quantitative signals.

\subsection{Ablation Study on Evolutionary Pressures}

To disentangle the roles of the three evolutionary pressures 
(selection, innovation, noise), we remove each component in turn 
and compare the resulting population dynamics 
(Figure~\ref{fig:ablation}). 
Without $\mathbf{V_{\mathrm{select}}}$ (left), competitive reinforcement vanishes 
and all agents remain at comparable proportions, producing a static, 
inefficient ecology. 
Without $\mathbf{V_{\mathrm{innovate}}}$ (middle), diversity collapses as FinCon and Trading 
rapidly dominate, leading to an oligopolistic lock-in. 
Without $\mathbf{V_{\mathrm{noise}}}$ (right), dynamics become smoother but rigid: 
FinCon and Trading still dominate, while adaptive reorganization is muted. 
Overall, selection drives efficiency, innovation sustains diversity, 
and noise acts as a perturbation amplifier that prevents premature lock-in 
and enables regime shifts.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/ablation_population.jpeg}
    \caption{Ablation study of evolutionary pressures. 
    From left to right: removing \emph{selection}, \emph{innovation}, and \emph{noise}.}
    \label{fig:ablation}
\end{figure}

\begin{table}[htbp]
\centering
\caption{Summary of ablation effects on market ecology.}
\label{tab:ablation_summary}
\begin{tabular}{lccc}
\toprule
 & \textbf{Diversity} & \textbf{Efficiency} & \textbf{Dynamic Reorganization} \\
\midrule
\textbf{No Innovate} & $\downarrow$ Collapse & $\uparrow$ Efficient oligopoly & $\downarrow$ Locked-in \\
\textbf{No Select}   & $\uparrow$ Preserved & $\downarrow$ Inefficient & $\downarrow$ Static \\
\textbf{No Noise}    & $\approx$ Moderate   & $\uparrow$ Stable & $\downarrow$ Rigid, no regime shift \\
\bottomrule
\end{tabular}
\end{table}

==> sections/3.tex <==
\iffalse
\section{Ecological Market Simulation Framework}

To instantiate the ecological game paradigm, we build a modular agent-based simulation platform that enables systematic, reproducible benchmarking of financial strategies in interactive, evolving markets.

\paragraph{Market Environment.}
We simulate a discrete-time market for a synthetic asset. At each round $t$, $N$ agents simultaneously submit buy/sell/hold orders, each with volume $v_i^t$ (subject to capital and position constraints).  
The market price is updated by a clearing mechanism that reflects the true balance of supply and demand:
\begin{equation}
P_{t+1} = P_t + \lambda \cdot \frac{\sum_{i} o_i^t v_i^t}{V_0 + \sum_{i} |v_i^t|} + \epsilon_t
\end{equation}
where $o_i^t = +1$ (buy), $-1$ (sell), $0$ (hold), $\lambda$ is the price impact factor, $V_0$ a liquidity regularizer, and $\epsilon_t \sim \mathcal{N}(0, \sigma_\epsilon^2)$ models exogenous noise (zero-sum if $\epsilon_t=0$).

\paragraph{Agent Library and Initialization.}
Agents are initialized from a diverse set of behavioral archetypes, each characterized by distinct decision rules:
\begin{itemize}
    \item \textbf{Trend-following}: $a_i^t = \text{buy}$ if $P_t > P_{t-1}$, $\text{sell}$ otherwise.
    \item \textbf{Contrarian}: $a_i^t = \text{sell}$ if $P_t > P_{t-1}$, $\text{buy}$ otherwise.
    \item \textbf{Fundamentalist}: Trades based on deviation from a reference value $P^*$; buys if $P_t < P^* - \theta$, sells if $P_t > P^* + \theta$ for some threshold $\theta$.
    \item \textbf{Event-driven}: Switches position in response to exogenous event signals $e_t$.
    \item \textbf{Random}: Selects $a_i^t \in \{\text{buy},\, \text{sell},\, \text{hold}\}$ uniformly at random, providing market liquidity and background noise.
    \item \textbf{Adaptive}: Updates strategy parameters online, e.g., via reinforcement learning or rolling performance statistics.
\end{itemize}

Each agent is initialized with an initial capital $C_i^0$ and position $S_i^0$, as well as type-specific behavioral parameters (such as lookback window, risk aversion, or threshold $\theta$). Trading volume $v_i^t$ is constrained by available capital, position limits, and other risk controls.

\paragraph{Evaluation Metrics.}

\vspace{-0.8em}
\begin{table}[h!]
\renewcommand{\arraystretch}{1.25}
\centering
\begin{tabular}{l l}
\toprule
\textbf{Individual Metrics} & \textbf{Definition / Formula} \\
\midrule
Net Profit for agent $i$        & $C_i^T + S_i^T P_T - (C_i^0 + S_i^0 P_0)$ \\
Sharpe Ratio for agent $i$      & $\displaystyle\frac{\mathbb{E}[\Delta W_i^t]}{\mathrm{Std}[\Delta W_i^t]}$ \\
Max Drawdown for agent $i$      & $\max_{t \leq T} \left(\max_{s \leq t} W_i^s - W_i^t \right)$ \\
Survival Time for agent $i$     & $\max\{t : C_i^t > C_{\min}\}$ \\
\midrule
\textbf{Ecological Metrics} &  \\
\midrule
Strategy Diversity (Entropy)    & $H^t = -\sum_k x_k^t \log x_k^t$ \\
% Population Turnover Rate        & $T^t = \displaystyle\frac{|\{\text{agents replaced at } t\}|}{N}$ \\
% Innovation Frequency            & $I^t = \displaystyle\frac{|\{\text{mutant entrants at } t\}|}{N}$ \\
% System Price Volatility         & $\text{Vol}^T = \sqrt{\frac{1}{T-1}\sum_{t=1}^T (P_t - \bar{P})^2}$ \\
Covariance Matrix & $\text{Cov}(x_i, x_j) = \mathbb{E}[(x_i - \bar{x}_i)(x_j - \bar{x}_j)]$
 \\
Co-occurrence Matrix & $C_{ij} = \frac{1}{T} \sum_{t} \mathbf{1}_{\{x_i(t) > \theta \land x_j(t) > \theta\}}$
\\

\midrule
\textbf{Interaction Metrics} & \\
\midrule
Ecological Sensitivity ($k$) & $\mathbb{E}[\text{Profit}_k \mid \text{mix}] - \mathbb{E}[\text{Profit}_k \mid \text{isolation}]$ \\
Competition Matrix ($k,\ell$) & $\mathbb{E}[\text{Profit}_k \mid \ell \text{ present}] - \mathbb{E}[\text{Profit}_k \mid \ell \text{ absent}]$ \\
\bottomrule
\end{tabular}
\caption{Summary of individual, ecological, and interaction evaluation metrics used in the simulation. Here, $W_i^t = C_i^t + S_i^t P_t$ denotes agent $i$'s total wealth at $t$.}
\end{table}
\vspace{-0.8em}

\fi

==> sections/4.tex <==

\section{Evolutionary Dynamics Experiments}
\label{sec:dynamics}

\subsection{Experimental Setup}
We simulate a population of $N=1000$ traders, each adopting one of $K \in \{4, 8, 16\}$ available strategies. Strategy types include trend-following, mean-reversion, high-frequency volatility, and LLM-based signal detection. Each strategy's return $f_k(t)$ evolves as an Ornstein–Uhlenbeck process, capturing mean-reverting reward signals with stochastic fluctuations. Strategy shares $x_k(t)$ evolve via a stochastic differential equation (SDE) that incorporates performance-based selection, social adaptation, and environmental noise. All shares are normalized such that $\sum_k x_k(t) = 1$.

\subsection{Representative Evolutionary Patterns}
We observe that under default parameters, strategy shares exhibit dynamic turnover. Some strategies dominate temporarily before being replaced. The system shows non-trivial transitions and intermittent concentration, depending on initial conditions and noise level.

\subsection{Convergence and Diversity}
To assess whether the system stabilizes or remains dynamic, we track the Shannon entropy $H(t) = -\sum_k x_k(t)\log x_k(t)$ and the average share change $\Delta x(t) = \sum_k |x_k(t) - x_k(t-1)|$. In many settings, the system converges to a steady distribution of strategy shares with moderate diversity. Higher adaptation rate $\mu$ tends to preserve diversity longer, while large $\sigma$ can destabilize convergence.

\subsection{Parameter Sensitivity and Phase Transitions}
We vary adaptation strength $\mu$ and noise level $\sigma$ across a grid to explore the phase behavior of the system. Results indicate the existence of qualitative transitions: from stable equilibrium to chaotic oscillations, or from diverse coexistence to monopolistic dominance. These phase boundaries are governed by the interplay of selection, adaptation, and noise.

\subsection{Mechanism Ablation Studies}
To verify the necessity of each component in the evolutionary dynamics, we perform ablation by selectively disabling terms in the evolution SDE. Removing social adaptation leads to premature dominance; removing noise results in overly deterministic convergence; removing performance pressure halts directional evolution. All three forces are necessary to reproduce realistic evolutionary dynamics.

\section{Structural and Statistical Analysis of Strategy Ecology}
\label{sec:structure}

\subsection{Preprocessing Pipeline}
To analyze structural patterns, we preprocess the time series $\{x_k(t)\}$ and $\{f_k(t)\}$ using rolling windows and isometric log-ratio (ilr) transformation to account for the compositional nature of shares. We discard initial transients and use windows of size $W=200$ for statistical estimation.

\subsection{Dependency Among Strategy Shares}
We compute the empirical covariance and correlation matrices among strategy shares across time windows. The resulting matrices reveal clusters of positively correlated strategies that often rise and fall together, as well as pairs with negative correlation, suggesting substitutive or competitive relationships. These patterns indicate the presence of ecological niches or alliances.

\subsection{Dependency Among Strategy Returns}
To understand signal similarity, we analyze pairwise correlations among the return series $f_k(t)$. Some strategy types exhibit strong return co-movement, suggesting redundant information sources or shared risk factors. We also perform PCA to quantify the effective dimensionality of the return space.

\subsection{Return-Driven Share Dynamics}
To explore causal influence, we compute lagged cross-correlations and transfer entropy from return series $f_k(t)$ to subsequent share adjustments $x_k(t+\tau)$. We also estimate vector autoregressive models with exogenous inputs (VARX) and extract impulse response functions (IRFs), showing how sudden return shocks propagate to share dynamics.

\subsection{Multilayer Ecological Network}
We construct an integrated ecological graph of strategies, where nodes represent strategies and edges encode statistical relationships: covariance (competition/cooperation), mutual information (nonlinear dependency), and transfer entropy (causal flow). The resulting network exhibits modular community structure and highlights key hubs that mediate transitions.

\subsection{Systemic Insights and Implications}
Our analysis reveals that evolutionary strategy systems can self-organize into stable clusters under appropriate parameters. The balance of performance pressure and adaptation preserves diversity while allowing for dominance cycles. External noise plays a dual role—inducing fluctuations but also preventing premature convergence. These findings point toward the emergence of evolutionary stable strategy (ESS) configurations and inform the design of robust agent-based financial systems.
